Building a Noisy Audio Dataset to Evaluate Machine Learning Approaches for Automatic Speech Recognition Systems

Automatic speech recognition systems are part of people's daily lives, embedded in personal assistants and mobile phones, helping as a facilitator for human-machine interaction while allowing access to information in a practically intuitive way. Such systems are usually implemented using machine learning techniques, especially with deep neural networks. Even with its high performance in the task of transcribing text from speech, few works address the issue of its recognition in noisy environments and, usually, the datasets used do not contain noisy audio examples, while only mitigating this issue using data augmentation techniques. This work aims to present the process of building a dataset of noisy audios, in a specific case of degenerated audios due to interference, commonly present in radio transmissions. Additionally, we present initial results of a classifier that uses such data for evaluation, indicating the benefits of using this dataset in the recognizer's training process. Such recognizer achieves an average result of 0.4116 in terms of character error rate in the noisy set (SNR = 30).

==> asr.tex <==
\section{Automatic Speech Recognition Systems}
\label{sec:asr}


==> resumo.tex <==
{\raggedright 
\textbf{Abstract.} 
Automatic speech recognition systems are part of people's daily lives, embedded in personal assistants and mobile phones, helping as a facilitator for human-machine interaction while allowing access to information in a practically intuitive way.
Such systems are usually implemented using machine learning techniques, especially with deep neural networks. Even with its high performance in the task of transcribing text to speech, few works address the issue of its recognition in noisy environments and, normally, the datasets used do not contain noise audio examples, while only mitigating this issue, through techniques of data augmentation.
This work aims to present the process of building a dataset of noisy audios, in a specific case of degenerated audios due to electromagnetic interference, commonly present in radio transmissions. 
Additionally, we present initial results of a classifier that uses such data for evaluation, showing the benefit of using such a set from the recognition training process that achieves a result of $??$ in terms of character error rate.
}

\medskip \medskip
{\raggedright 
\textbf{Keywords}: Machine Learning, Datasets, Automatic Speech Recognition Systems, Noisy Audio.}

\medskip \medskip

{\raggedright 
\textbf{Resumo.} 
Sistemas de reconhecimento automático de fala fazem parte da vida cotidiana das pessoas, embutidos em assistentes pessoais e telefones celulares, auxiliando a funcionando como um facilitador para a interação homem-máquina ao mesmo tempo que permitem o acesso à informação de forma praticamente intuitiva.
Tais sistemas são normalmente implementados utilizando técnicas de aprendizado de máquina, especialmente com redes neurais profundas. Mesmo com o seu alto desempenho na tarefa de transcrever o texto da fala, poucos trabalhos endereçam a questão do seu reconhecimento em ambientes ruidosos e, normalmente, as bases utilizadas não apresentam exemplos de áudios ruídos, apenas mitigando tal questão, por intermédio de técnicas de aumentação de dados. 
Este trabalho tem por objetivo apresentar o processo de construção de uma base de dados de áudios ruidosos, em um caso específico de áudios degenerados em função de interferências eletromagnéticas, comumente presentes em transmissões rádio. Adicionalmente, apresentamos resultados iniciais de um classificador que utiliza tais dados para avaliação mostrando os benefícios de se utilizar tal conjunto já no processo de treinamento dos reconhecedores que alcança um resultado de $??$ em termos de taxa de erro de caracteres. 
}

\medskip \medskip

{\raggedright 
\textbf{Palavras-chave}: Aprendizado de Máquina, Conjuntos de Dados, Sistemas de Reconhecimento Automático de voz, Áudios Ruídosos.}
